Model Checking Embedded C Software using k-Induction and Invariants (extended version)

We present a proof by induction algorithm, which combines k-induction with invariants to model check embedded C software with bounded and unbounded loops. The k-induction algorithm consists of three cases: in the base case, we aim to find a counterexample with up to k loop unwindings; in the forward condition, we check whether loops have been fully unrolled and that the safety property P holds in all states reachable within k unwindings; and in the inductive step, we check that whenever P holds for k unwindings, it also holds after the next unwinding of the system. For each step of the k-induction algorithm, we infer invariants using affine constraints (i.e., polyhedral) to specify pre- and post-conditions. Experimental results show that our approach can handle a wide variety of safety properties in typical embedded software applications from telecommunications, control systems, and medical devices; we demonstrate an improvement of the induction algorithm effectiveness if compared to other approaches.

==> figuras/sum01.tex <==
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.5cm,
                    semithick]
   \tikzstyle{every state}=[rectangle,rounded corners=10pt]

  \node[initial,state] 		(A)                    {$init$};
  \node[state]         		(B) [below=0.8cm of A] {compute sn};
  \node[state]         		(C) [right of=B] {increment i};
  \node[state, accepting]	(D) [below=0.8cm of C] {terminate};

   \path (A) edge [left]	node {$n \geq 1$} (B)
         (B) edge [bend left]	node {$ \tau $} (C)
	 (C) edge [bend left]	node {$i \leq n$} (B)
	     edge		node {$i > n$} (D);
\end{tikzpicture}


==> figuras/sum01_bug.tex <==
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.5cm,
                    semithick]
   \tikzstyle{every state}=[rectangle,rounded corners=10pt]

  \node[initial,state] 		(A)                    {$init$};
  \node[state]         		(B) [below of=A] {compute sn};
  \node[state]         		(C) [right of=B] {increment i};
  \node[state, accepting]	(D) [below of=C] {terminate};

   \path (A) edge [left]	node {$n \geq 1 \wedge i < 10$} (B)
         (B) edge [bend left]	node {$ \tau $} (C)
	 (C) edge [bend left]	node {$i < 10$} (B)
	     edge		node {$i > n$} (D)
	     edge [loop right]	node {$i \geq 10$} ();
\end{tikzpicture}


==> figuras/sum01_bug_kripke.tex <==
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.5cm,
                    semithick]
   \tikzstyle{every state}=[rectangle,rounded corners=10pt]

  \node[initial,state] (A)              {$1, ?, 0$};
  \node[state]         (B) [below of=A] {$i_n, n, sn$};
  \node[state]         (C) [below left of=B] {$i_{n+1}, n, sn+2$};
  \node[state]         (D) [below right of=B] {$i_{n+1}, n, sn$};
  \node[state]         (E) [below of=C] {$n+1, n, sn$};
  \node[state]         (F) [below of=D] {$n+1, n, 18$};
  \node[state]         (G) [below left of=E] {$n+1, n, 0$};
  \node[state]         (H) [below right of=E] {$n+1, n, n\times2$};

   \path (A) edge              node {} (B)
         (B) edge [pos=0.6]    node {$i < 10$} (C)
	     edge [left, pos=0.8]      node {$i \geq n$} (D)
         (C) edge [bend left]  node {$i \leq n$} (B)
             edge [left]       node {$i>n$} (E)
         (D) edge              node {$i>n$} (F)
             edge [bend right, right] node {$n \neq 0$} (B)
         (E) edge [left, pos=0.3]       node {$n=0$} (G)
             edge [right,pos=0.3]       node {$n \neq 0$} (H);
\end{tikzpicture}


==> figuras/sum01_kripke.tex <==
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.5cm,
                    semithick]
   \tikzstyle{every state}=[rectangle,rounded corners=10pt]

  \node[initial,state] (A)                    {$1, ?, 0$};
  \node[state]         (B) [below of=A] {$i_n, n, sn$};
  \node[state]         (C) [right of=B] {$i_{n+1}, n, sn+2$};
  \node[state]         (D) [below of=B] {$n+1, n, sn$};
  \node[state]         (F) [below right of=D] {$n+1, n, 0$};
  \node[state]         (E) [below left of=D] {$n+1, n, n\times2$};

   \path (A) edge              node {} (B)
         (B) edge              node {$i > n$} (D)
	 (B) edge [bend left]  node {$i \leq n$} (C)
         (C) edge [bend left]  node {} (B)
         (D) edge [left]       node {$n=0$} (E)
         (D) edge [right]      node {$n \neq 0$} (F);
\end{tikzpicture}

